The Power of The Hybrid Model for Mean Estimation

We explore the power of the hybrid model of differential privacy (DP), in which some users desire the guarantees of the local model of DP and others are content with receiving the trusted-curator model guarantees. In particular, we study the utility of hybrid model estimators that compute the mean of arbitrary real-valued distributions with bounded support. When the curator knows the distribution's variance, we design a hybrid estimator that, for realistic datasets and parameter settings, achieves a constant factor improvement over natural baselines. We then analytically characterize how the estimator's utility is parameterized by the problem setting and parameter choices. When the distribution's variance is unknown, we design a heuristic hybrid estimator and analyze how it compares to the baselines. We find that it often performs better than the baselines, and sometimes almost as well as the known-variance estimator. We then answer the question of how our estimator's utility is affected when users' data are not drawn from the same distribution, but rather from distributions dependent on their trust model preference. Concretely, we examine the implications of the two groups' distributions diverging and show that in some cases, our estimators maintain fairly high utility. We then demonstrate how our hybrid estimator can be incorporated as a sub-component in more complex, higher-dimensional applications. Finally, we propose a new privacy amplification notion for the hybrid model that emerges due to interaction between the groups, and derive corresponding amplification results for our hybrid estimators.

==> future_work.tex <==
\paragraph*{Future Work}
One direction for future work is determining whether the hybrid model is strictly more powerful than its composing models.
One way to determine this is to prove that a hybrid model algorithm has uniformly higher utility than optimal non-hybrid baselines.
In this work, we didn't answer this question since our baselines aren't necessarily optimal.
Instead, we chose our baselines because they are common in practice and enabled us to derive exact finite-sample utility expressions.
Concurrently with this work, Beimel et al.~\cite{beimel2020power} have undertaken another approach to affirmatively show that, for a selection of theoretical problems, the hybrid model is strictly more powerful.
However, for applied problems more complex than univariate mean estimation, quantifying the power of the hybrid model remains an open question.

Another important direction is further exploring the role of inter-group interactivity.
Avent et al.~\cite{blender} experimentally showed that it is possible for one group to intelligently provide information to the other in order to increase the utility, and Beimel et al.~\cite{beimel2020power} theoretically showed that inter-group interactivity is sometimes necessary for the hybrid model to be more powerful than its composing models.
However, in this work, we showed that the Avent et al.'s interaction strategy enables no privacy amplification.
Additionally, we proved that it is possible to amplify users' privacy guarantees without exchanging information between groups -- although we did so without exploring how this lack of interaction may affect utility.
This opens a new line of research in the hybrid model: the privacy--utility trade-off arising from inter-group interactivity.
Moreover, it is possible that this privacy amplification isn't always equal for both groups.
This motivates a natural generalization of the hybrid model where a user's choice between groups isn't based only on their trust preferences, but also on the DP guarantee provided.
Viewed through a game-theoretic lens, users could be modeled as rational agents whose goal is to optimize their personal utility, which would be a function that takes into account their group choice and corresponding DP guarantee.
Mechanisms could then be designed to align users' incentives with the analyst's utility goal.


==> nwh.tex <==
\section{NWH Estimator (Homogeneous Setting)} \label{app:nwh}
The weighting scheme we explore here gives us the ``na\"{\i}vely-weighted hybrid'' (NWH) estimator, as this is the weighting one would choose in the non-private setting: weight all user's data equally, not taking into account the difference in privacy errors between the two groups of users.
This is equivalent to minimizing the excess sampling error (or rather, ensuring $0$ excess sampling error at the expense of uncontrolled privacy error).
Explicitly, this corresponds to setting $w = c$ in Definition~\ref{def:hybrid}, yielding the following estimator.

\begin{defn} \label{def:nwh}
The na\"{\i}vely-weighted hybrid estimator is:
$$\tilde{\mu}_{NWH} = c\tilde{\mu}_T + (1-c)\tilde{\mu}_L.$$
\end{defn}

\begin{lem} \label{lem:nwh-mse}
The na\"{\i}vely-weighted hybrid estimator, $\tilde{\mu}_{NWH}$, has expected squared error:
$$\mathcal{E}_{NWH} = c^2 s_T^2 + \frac{(1-c)}{n}s_L^2.$$
\end{lem}

\noindent Note that there is no excess sampling error, just privacy error that is dependent on the fraction of users in each model.
Thus, we can intuitively expect reasonable performance from this estimator when the privacy variance is dwarfed by the data variance $\sigma^2$ (since this indirectly optimized for the data variance); otherwise, we'd expect this estimator to perform poorly.

Here, we compute and analyze the relative improvement in MSE of the na\"{\i}vely-weighted hybrid estimator relative to the MSEs of the TCM-Only estimator and the Full-LM estimator.

\begin{thm}
The relative improvement of the NWH estimator $\tilde{\mu}_{NWH}$ over the better of $\tilde{\mu}_T$ and $\tilde{\mu}_F$ is:
\begin{equation*}
R(\mathcal{E}_{NWH}) = \gamma \cdot
\begin{cases}
	\frac{1-c}{cn}\sigma^2 + s_T^2 & \text{if $c>c_{crit} \wedge n \le n_{crit}$} \\
	\frac{s_L^2}{n} & \text{otherwise}
  \end{cases},
\end{equation*}
where $\gamma = \frac{n}{c^2 n s_T^2+(1-c) s_L^2}$ and $c_{crit}$ and $n_{crit}$ are as defined in Definition~\ref{def:R-crit}.
\end{thm}
\begin{proof}
Direct application of Lemmas~\ref{lem:tcm-only-mse}, \ref{lem:full-lm-mse}, and~\ref{lem:nwh-mse} to Definition~\ref{def:R-crit}.
\end{proof}

Unlike the relative improvement of the estimator in the known-variance case, $R(\mathcal{E}_{KVH}) \ge 1$ cannot be guaranteed over the entire space of parameters.
The region in which this does hold is complex and difficult to obtain, so we instead turn our focus to the relative improvement over the worse of the two baselines.

\begin{thm}
The relative improvement of the NWH estimator $\tilde{\mu}_{NWH}$ over the worse of $\tilde{\mu}_T$ and $\tilde{\mu}_F$ is:
\begin{equation*}
r(\mathcal{E}_{NWH}) = \gamma \cdot
\begin{cases}
	\frac{s_L^2}{n} & \text{if $c>c_{crit} \wedge n \le n_{crit}$} \\
	\frac{1-c}{cn}\sigma^2 + s_T^2 & \text{otherwise}
  \end{cases},
\end{equation*}
where $\gamma = \frac{n}{c^2 n s_T^2+(1-c) s_L^2}$ and $c_{crit}$ and $n_{crit}$ are as defined in Definition~\ref{def:R-crit}.
\end{thm}
\begin{proof}
Direct application of Lemmas~\ref{lem:tcm-only-mse}, \ref{lem:full-lm-mse}, and~\ref{lem:nwh-mse} to Definition~\ref{def:r-crit}.
\end{proof}

Indeed, we have for this relative improvement measure for $\tilde{\mu}_{NWH}$ that $r(\mathcal{E}_{NWH}) \ge 1$ over the entire space of parameters.

\begin{figure*}[h]
\centering
\begin{tabular}{ccc}
  \includegraphics[width=.33\linewidth]{figs/beta_low_var_R_homo_nwh.pdf} &  \includegraphics[width=.33\linewidth]{figs/beta_med_var_R_homo_nwh.pdf} &
  \includegraphics[width=.33\linewidth]{figs/beta_high_var_R_homo_nwh.pdf}\\
(a) & (b) & (c) \\
 \includegraphics[width=.33\linewidth]{figs/beta_low_var_rr_homo_nwh.pdf} &   \includegraphics[width=.33\linewidth]{figs/beta_med_var_rr_homo_nwh.pdf} &
 \includegraphics[width=.33\linewidth]{figs/beta_high_var_rr_homo_nwh.pdf} \\
(d) & (e) & (f) \\
\end{tabular}
\caption{Across a range of $n$ values, for various $c$ and $\epsilon$ values for each Beta distribution (plotted in Figure~\ref{fig:beta-R-kvh}a): (a,b,c) shows $R(\mathcal{E}_{NWH})$ values and (d,e,f) shows $r(\mathcal{E}_{NWH})$ values.}
\label{fig:beta-nwh}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{tabular}{cc}
  \includegraphics[width=.45\linewidth]{figs/salary_heatmap_R_homo_nwh.pdf} &  \includegraphics[width=.45\linewidth]{figs/salary_heatmap_rr_homo_nwh.pdf} \\
(a) & (b) \\
\end{tabular}
\caption{The relative improvements $R(\mathcal{E}_{NWH})$ (a) and  $r(\mathcal{E}_{NWH})$ (b) across a range of $c$ and $\epsilon$ values.}
\label{fig:uc-salary-nwh}
\end{figure*}


\subsection{Empirical Evaluation of $R(\mathcal{E}_{NWH})$ and $r(\mathcal{E}_{NWH})$} \label{sec:exploring-nwh}

Here, we explore both relative improvement measures $R(\mathcal{E}_{NWH})$ and $r(\mathcal{E}_{NWH})$ using the $\epsilon$-DP Laplace mechanism in the context of several datasets (described in Section~\ref{sec:exploring-R-kvh}).

Figure~\ref{fig:beta-nwh} presents $R(\mathcal{E}_{NWH})$ (top row) and $r(\mathcal{E}_{NWH})$ (bottom row) using the various Beta distributions.
For each distribution, the relative improvement measures are plotted across $n \in [10^3, 10^5]$, for parameters $c \in \{0.5\%, 5\%\}$ and $\epsilon \in \{0.1, 1\}$.
From the top row of the figure, we find that there are several regions where $R(\mathcal{E}_{NWH})$ achieves a value just greater than $1$.
Most regions, however, yield $R(\mathcal{E}_{NWH})$ significantly less than $1$.
While this indicates that $\tilde{\mu}_{NWH}$ is worse in those regions than the better of the two baseline estimators, we turn to the bottom row of the figure to understand how much better it is than the worse of the baselines.
Focusing on the regions where $R(\mathcal{E}_{NWH})$, we see that the $r(\mathcal{E}_{NWH})$ values, while always greater than $1$, are not significantly greater.

Figure~\ref{fig:uc-salary-nwh} presents heatmaps of $R(\mathcal{E}_{NWH})$ and $r(\mathcal{E}_{NWH})$ for the UC salaries dataset.
Recall that $n$, $m$, and $\sigma$ are determined by this dataset, so for the remaining free parameters, we explore: $c \in [0.1\%, 10\%]$ and $\epsilon \in [0.1, 10]$.
We find that $R(\mathcal{E}_{NWH})$ achieves a value of slightly greater than $1$ across a large portion of the space.
However, as expected, there is also a significant portion of the space where $R(\mathcal{E}_{NWH})$ was less than $0.2$.
We also find that $r(\mathcal{E}_{NWH})$ achieves greater than 1 in the entire region, although less than $5$ in most of it.
However, there is a small region where $c$ is large that $r(\mathcal{E}_{NWH})$ exceeds $20$.

Taken together, these results indicate that na\"{\i}ve-weighting may not be the best heuristic, despite this estimator having some regions where it performs competitively against the best of the baseline estimators.
Thus, we now consider a more intelligent weighting heuristic.

\subsection{Comparing $\tilde{\mu}_{NWH}$ and $\tilde{\mu}_{PWH}$}
Comparing the evaluations of the relative improvement of $\tilde{\mu}_{NWH}$ (Section~\ref{sec:exploring-nwh}) and of $\tilde{\mu}_{PWH}$ (Section~\ref{sec:exploring-pwh}), it is clear that for most practical applications where variance is not known, $\tilde{\mu}_{PWH}$ is the superior estimator.
Not only was it often able to have superior utility to the better of the two baselines, but in some regions, it had utility competitive with the known-variance estimator.
One drawback is that, due to the complexity of its weighting scheme (relative to the na\"{\i}ve weighting scheme), we were unable to analytically obtain the regions where $R(\mathcal{E}_{PWH}) > 1$ is guaranteed for the generic class of noise-addition mechanisms (although we were able to do so for the specific case of the Laplace mechanism).
Overall though, $\tilde{\mu}_{PWH}$ seems to be the superior hybrid estimator for practical purposes when the variance is unknown.

